The Alignment Paradox: How Post-Training Amplifies Confident Hallucinations in Language Models

Large language models (LLMs) can produce factually incorrect answers with high confidence, undermining their reliability and limiting the effectiveness of uncertainty-based error detection. While prior research attributes confident hallucinations to factors such as missing knowledge in training data, reasoning errors, or stochastic decoding, we uncover that post-training alignment itself is a primary driver of these errors, a phenomenon we call the \textbf{Alignment Paradox}. Across five model families evaluated on factual benchmarks, unaligned base models produce few high-confidence errors on long-tail factual queries, whereas instruction-tuned models multiply high-confidence errors ($p \ge 0.95$) by more than an order of magnitude (10$\times$ to 35$\times$). Layer-wise probing with the Logit Lens reveals that this overconfidence emerges in late layers, where wrong-answer margins expand past 4.0 points after remaining near zero across early and intermediate layers. These findings motivate limiting margin growth during post-training. We implement this principle through an entropy-dependent margin bound in direct preference optimization (DPO). In multi-epoch experiments with Mistral-7B, the bounded objective reduces high-confidence errors by up to 35.3\% relative to standard DPO while maintaining performance on evaluated general reasoning benchmarks. These results show that bounded margins mitigate confident hallucinations during post-training.

==> hce_arxiv/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation (avoid using if possible)
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> hce_arxiv/sections/00_abstract.tex <==
\begin{abstract}
Large language models (LLMs) can produce factually incorrect answers with high confidence, undermining their reliability and limiting the effectiveness of uncertainty-based error detection. While prior research attributes confident hallucinations to factors such as missing knowledge in training data, reasoning errors, or stochastic decoding, we uncover that post-training alignment itself is a primary driver of these errors, a phenomenon we call the \textbf{Alignment Paradox}. Across five model families evaluated on factual benchmarks, unaligned base models produce few high-confidence errors on long-tail factual queries, whereas instruction-tuned models multiply high-confidence errors ($p \ge 0.95$) by more than an order of magnitude (10$\times$ to 35$\times$). Layer-wise probing with the Logit Lens reveals that this overconfidence emerges in late layers, where wrong-answer margins expand past 4.0 points after remaining near zero across early and intermediate layers. These findings motivate limiting margin growth during post-training. We implement this principle through an entropy-dependent margin bound in direct preference optimization (DPO). In multi-epoch experiments with Mistral-7B, the bounded objective reduces high-confidence errors by up to 35.3\% relative to standard DPO while maintaining performance on evaluated general reasoning benchmarks. These results show that bounded margins mitigate confident hallucinations during post-training.
\end{abstract}


==> hce_arxiv/sections/01_introduction.tex <==
\section{Introduction}
\label{sec:intro}

When large language models produce errors with low confidence ($p \approx 0.3\text{--}0.5$), uncertainty-based error detection and selective prediction \citep{geifman2017selective} can reliably flag or defer the query. A critical vulnerability arises when models produce incorrect assertions with high confidence ($p \ge 0.95$). Such confident hallucinations evade threshold-based abstention, bypass automated verification, and undermine decision systems where abstention is preferable to erroneous completions \citep{amodei2016concrete,kadavath2022language}.

While prior research attributes factual hallucinations to pre-training knowledge gaps, multi-step reasoning errors, or decoding noise \citep{kadavath2022language,dziri2023faith,chuang2024dola,orgad2025llms}, post-training alignment, comprising supervised fine-tuning (SFT; \citealt{ouyang2022training}) and preference optimization \citep{bai2022training,rafailov2023direct}, is widely assumed to improve truthfulness and safety \citep{touvron2023llama,dubey2024llama,qwen2024technical}. In this work, we uncover that post-training alignment itself is a primary driver of high-confidence errors, a phenomenon we term the \textbf{Alignment Paradox}\footnote{Code and evaluation data are accessible at \url{https://github.com/star5o/HCE}.}. Although alignment enhances conversational adherence, it degrades confidence reliability on factual queries, shifting incorrect predictions into extreme confidence regimes ($p \ge 0.95$).

\begin{figure}[t]
\centering
\includegraphics[width=0.88\textwidth]{figs/fig0_overview.pdf}
\caption{\textbf{The Alignment Paradox.} Post-training alignment shifts output probabilities into high-confidence regimes and multiplies near-certain errors on factual queries. (a) Sequence confidence distributions on factual queries (\texttt{Mistral-7B}). (b) Progression of high-confidence error rates ($p \ge 0.95$) and first-token decision entropy across alignment stages in the \texttt{LLaMA-3.1-8B} lineage (Base $\to$ SFT $\to$ DPO $\to$ RLVR). (c) Layer-wise logit margin across normalized depth, showing logit margin expansion in late layers ($l/L \ge 0.85$, \texttt{Mistral-7B}).}
\label{fig:overview}
\vspace{-4pt}
\end{figure}

Empirical evaluation demonstrates this phenomenon across standard factual question-answering benchmarks. As illustrated in Figure~\ref{fig:overview}a, when an unaligned base model encounters an entity absent from its parametric memory, its output distribution remains diffuse across competing candidates, reflecting epistemic uncertainty. In contrast, post-trained checkpoints exhibit pronounced probability concentration, assigning probabilities exceeding $0.95$ even to false entities. Across five matched base and aligned model pairs spanning 7B to 14B parameters in the Mistral, Qwen, and LLaMA lineages over 22,267 factual queries, post-training alignment multiplies high-confidence errors ($p \ge 0.95$) by 10.0$\times$ to 35.4$\times$, worsening Expected Calibration Error (ECE; \citealt{guo2017calibration}) by up to 15.5-fold.

To determine whether this surge reflects conversational chat templates, we evaluate aligned models on bare completion prompts identical to those used for base models. Parameter updates account for the vast majority of the increase, as aligned checkpoints retain a 4.1$\times$ to 6.0$\times$ elevation in confident errors over base models even in the absence of instruction formatting. Furthermore, tracking sequential checkpoints across post-training reveals a two-stage progression, where supervised fine-tuning contracts decision entropy and preference optimization expands logit margins, driving incorrect outputs into extreme confidence intervals.

To investigate internal mechanisms, we probe intermediate representations using the Logit Lens \citep{belrose2023eliciting}. Our analysis shows that early commitment does not extend to factual errors, as decision distributions remain diffuse across early and intermediate representations. Overconfidence emerges strictly in late layers ($l/L \ge 0.85$), where wrong-answer margins expand past 4.0 points after hovering near zero through earlier layers, sharply suppressing decision entropy.

Inference-time interventions provide limited mitigation. Across five representative test-time defenses (defensive prompting, two-turn self-correction, sampling self-consistency, layer-contrastive decoding with DoLa \citep{chuang2024dola}, and entropy thresholding), we find that these heuristics eliminate at most 5\% to 8\% of high-confidence errors while preserving at least 97\% of correct completions. Furthermore, iterative self-correction degrades accuracy on initially correct completions. Because test-time heuristics cannot reverse parameter-level margin expansion, mitigating confident hallucinations requires regularizing the training objective itself.

We address this challenge by establishing the principle of bounded margin optimization for post-training alignment. Grounded in theoretical analysis showing that standard preference objectives drive logit margins toward infinity on ungrounded completions, we demonstrate that constraining margin expansion provides a general remedy against ungrounded overconfidence. We formulate Bounded Dynamic Margin (BDM) optimization, which enforces an adaptive, entropy-dependent ceiling on margin growth. During standard optimization on supported preferences, the margin bound remains inactive; under extended optimization on unsupported completions, it activates to prevent unbounded logit expansion. In multi-epoch evaluations across 22,267 factual queries, instantiating this principle via BDM-DPO reduces high-confidence errors by up to 35.3\% relative to standard DPO (eliminating 850 confident errors) while preserving general reasoning capabilities.

In summary, this work presents four primary contributions.
\begin{enumerate}
    \item \textbf{The Alignment Paradox.} We formalize the empirical phenomenon wherein post-training alignment multiplies high-confidence factual errors by 10.0$\times$ to 35.4$\times$ across five model families while degrading confidence reliability.
    \item \textbf{Causal Attribution.} Through prompt ablations and checkpoint tracking, we demonstrate that parameter updates rather than chat templates drive this effect, with preference objectives expanding logit margins on erroneous completions.
    \item \textbf{Representation Dynamics.} Using layer-wise Logit Lens probing, we show that early commitment does not hold for factual errors, demonstrating that overconfidence emerges strictly in late layers ($l/L \ge 0.85$).
    \item \textbf{Principled Mitigation.} We show that test-time defenses achieve at most an 8.3\% error reduction, and establish that constraining margin expansion provides a general training-time remedy. Instantiated as BDM-DPO, this bounded formulation reduces high-confidence errors by up to 35.3\% while preserving general reasoning performance.
\end{enumerate}


==> hce_arxiv/sections/02_related_work.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{Factual Knowledge and Confidence Reliability.}
Evaluating factual accuracy in large language models spans diverse benchmarks, including TruthfulQA \citep{lin2021truthfulqa}, PopQA \citep{mallen2023when}, TriviaQA \citep{joshi2017triviaqa}, and Natural Questions \citep{kwiatkowski2019natural}. Standard evaluation protocols traditionally aggregate all incorrect generations into an undifferentiated error rate, treating an uncertain error ($p \approx 0.35$) identically to an authoritative fabrication ($p \ge 0.95$). In high-stakes settings relying on selective abstention \citep{geifman2017selective,kamath2020selective,kadavath2022language}, these modes differ fundamentally, because uncertain errors trigger human review, whereas near-certain errors invisibly bypass confidence filters. While confidence reliability metrics such as Expected Calibration Error (ECE; \citealt{guo2017calibration}) and Brier score \citep{brier1950verification} are established \citep{desai2020calibration,xiong2024can}, prior studies focus on static evaluations, lacking systematic frameworks to track how post-training pipelines alter confidence geometry.

\paragraph{Mechanistic Probing of Factual Recall.}
Mechanistic interpretability has made rapid progress in tracing factual associations in transformer layers \citep{meng2022locating,geva2023dissecting}. Linear probing and activation steering methods \citep{azaria2023internal,burns2023discovering,li2024inference,orgad2025llms} show that intermediate activations often separate true assertions from falsehoods. Complementary work investigates self-detection heads \citep{kadavath2022language,yin2023large}, entity familiarity estimation \citep{ferrando2025do}, and layer-contrastive decoding such as DoLa \citep{chuang2024dola}. However, these studies typically treat base and aligned models as fixed entities, without tracing the causal transition from pre-training to post-training representations or elucidating how instruction tuning reshapes internal uncertainty manifolds.

\paragraph{Preference Optimization and Alignment Dynamics.}
Direct preference optimization (DPO; \citealt{rafailov2023direct}) and related variants (IPO \citep{azar2024general}, KTO \citep{ethayarajh2024kto}, SimPO \citep{meng2024simpo}, and reinforcement learning with verifiable rewards (RLVR; \citealt{shao2024deepseekmath})) have largely supplanted reinforcement learning from human feedback based on PPO \citep{christiano2017deep,stiennon2020learning,ouyang2022training}. While enforcing conversational compliance, their susceptibility to reward over-optimization has attracted scrutiny \citep{gao2023scaling,singhal2024long,coste2024reward}. Most investigations into post-training capability trade-offs focus on core reasoning degradation on math or code benchmarks \citep{ouyang2022training,dubey2024llama}. In contrast, our work examines an epistemic dimension, demonstrating how unconstrained preference margins force steep entropy compression on factual queries, converting benign uncertainty into confident hallucinations.


==> hce_arxiv/sections/03_paradox_evidence.tex <==
\section{Empirical Evidence for the Alignment Paradox}
\label{sec:empirical}

\subsection{Evaluation Setup and Reliability Metrics}
\label{sec:setup}

To evaluate how post-training alignment alters factual certainty, we benchmark five matched base and instruction-tuned model pairs across 22,267 factual queries. The evaluation spans the Mistral, Qwen, and LLaMA lineages across 7B to 14B parameter scales, specifically Mistral-7B \citep{jiang2023mistral}, Qwen3-8B and Qwen3-14B \citep{qwen2024technical}, LLaMA-3.1-8B \citep{dubey2024llama}, and Mistral-Nemo-12B. We evaluate on PopQA (12,509 open-domain queries; \citealt{mallen2023when}) and TriviaQA (9,758 unfiltered validation queries; \citealt{joshi2017triviaqa}), complemented by Natural Questions \citep{kwiatkowski2019natural} for broader consistency checks.

We enforce deterministic greedy decoding ($T=0$) to eliminate sampling variance. Generated strings are evaluated using regular expression word-boundary matching against verified reference aliases from Wikidata (Appendix~\ref{app:protocols}; checkpoint specifications appear in Table~\ref{tab:app_model_specs}, and double-blind audits confirming over 98.6\% hallucination fidelity appear in Table~\ref{tab:app_human_audit_breakdown}). For each query, we track the sequence geometric mean probability $\bar{p}$ and Expected Calibration Error (ECE; \citealt{guo2017calibration}) across $M=10$ bins:
\begin{equation}
\bar{p} = \exp\left( \frac{1}{T} \sum_{t=1}^T \ln p(y_t \mid x, y_{<t}) \right), \qquad \text{ECE} = \sum_{m=1}^M \frac{|B_m|}{N} \left| \text{acc}(B_m) - \text{conf}(B_m) \right|
\label{eq:metrics}
\end{equation}
where $B_m$ denotes samples in bin $m$, and $\text{acc}(B_m)$ and $\text{conf}(B_m)$ denote empirical accuracy and mean confidence. Under a selective prediction threshold $\tau = 0.95$, we stratify outputs into four quadrants, denoted as \textbf{Gate A} ($\bar{p} \ge 0.95$, correct), \textbf{Gate B} ($\bar{p} \ge 0.95$, incorrect; confident hallucinations), \textbf{Gate C} ($\bar{p} < 0.95$, incorrect), and \textbf{Gate D} ($\bar{p} < 0.95$, correct).

\begin{table}[t]
\centering
\small
\caption{\textbf{Base versus aligned models across 22,267 queries.} Post-training alignment multiplies high-confidence errors (Gate B) and degrades confidence reliability.}
\label{tab:main_results}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccc}
\toprule
\textbf{Model Family} & \textbf{Checkpoint} & \textbf{Acc (\%)} & \textbf{Gate A} & \textbf{Gate B} & \textbf{Ratio} & \textbf{Gate C} & \textbf{Gate D} & \textbf{ECE} \\
\midrule
\multirow{2}{*}{Mistral-7B} & Base & 52.3 & 2,378 (10.7\%) & 97 (0.4\%) & \multirow{2}{*}{\textbf{14.1$\times$}} & 10,525 (47.3\%) & 9,256 (41.6\%) & 0.097 \\
 & Instruct & 41.6 & 4,133 (18.6\%) & 1,366 (6.1\%) & & 11,605 (52.1\%) & 5,125 (23.0\%) & 0.378 \\
\midrule
\multirow{2}{*}{Qwen3-8B} & Base & 45.9 & 1,885 (8.5\%) & 50 (0.2\%) & \multirow{2}{*}{\textbf{35.4$\times$}} & 11,986 (53.9\%) & 8,318 (37.4\%) & 0.042 \\
 & Instruct & 37.9 & 5,140 (23.1\%) & 1,768 (7.9\%) & & 11,993 (53.9\%) & 3,308 (14.9\%) & 0.400 \\
\midrule
\multirow{2}{*}{LLaMA-3.1-8B} & Base & 55.3 & 1,406 (6.3\%) & 38 (0.2\%) & \multirow{2}{*}{\textbf{15.7$\times$}} & 9,909 (44.5\%) & 10,910 (49.0\%) & 0.018 \\
 & Instruct & 45.6 & 4,996 (22.4\%) & 596 (2.7\%) & & 11,494 (51.6\%) & 5,157 (23.2\%) & 0.262 \\
\midrule
\multirow{2}{*}{Mistral-Nemo-12B} & Base & 57.7 & 1,690 (7.6\%) & 56 (0.3\%) & \multirow{2}{*}{\textbf{10.0$\times$}} & 9,367 (42.1\%) & 11,150 (50.1\%) & 0.017 \\
 & Instruct & 47.6 & 4,766 (21.4\%) & 560 (2.5\%) & & 11,092 (49.8\%) & 5,834 (26.2\%) & 0.264 \\
\midrule
\multirow{2}{*}{Qwen3-14B} & Base & 51.0 & 2,727 (12.5\%) & 104 (0.5\%) & \multirow{2}{*}{\textbf{19.8$\times$}} & 10,564 (48.5\%) & 8,391 (38.5\%) & 0.066 \\
 & Instruct & 43.4 & 6,727 (30.2\%) & 2,061 (9.3\%) & & 10,451 (46.9\%) & 2,938 (13.2\%) & 0.371 \\
\bottomrule
\end{tabular}%
}
\end{table}

\subsection{Post-Training Alignment Multiplies High-Confidence Errors}
\label{sec:findings}

Table~\ref{tab:main_results} presents the primary empirical finding. Across every model family, unaligned base models rarely produce high-confidence errors on factual queries; out of 22,267 queries, base models produce only 38 to 104 Gate B errors (0.2\% to 0.5\%). The vast majority of base errors fall into Gate C, where low probabilities accurately signal lack of knowledge.

Post-training alignment significantly alters this behavior. On identical queries, confident errors expand by 10.0$\times$ to 35.4$\times$ across all five families, rising to 1,768 in Qwen3-8B (35.4$\times$), 1,366 in Mistral-7B (14.1$\times$), and 2,061 in Qwen3-14B (19.8$\times$). Simultaneously, confidence reliability degrades as instruction-tuned models develop severe overconfidence, driving Expected Calibration Error (ECE) up by up to 15.5-fold (from 0.017 to 0.264 in Mistral-Nemo-12B, and 0.018 to 0.262 in LLaMA-3.1-8B).

\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/fig1_reliability.pdf}
    \caption{Reliability diagram.}
    \label{fig:reliability}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/fig2_pbar_dist.pdf}
    \caption{Confidence distribution ($\bar{p}$).}
    \label{fig:pbar_dist_main}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/fig6_strata_panel.pdf}
    \caption{Entity popularity tiers.}
    \label{fig:pop_tiers}
\end{subfigure}
\caption{\textbf{Confidence reliability and distribution dynamics across 22,267 queries.} (a) Reliability diagrams show post-training overconfidence gaps. (b) Sequence confidence distributions ($\bar{p}$) reveal that unaligned base errors remain in the low-confidence regime, whereas post-training alignment drives thousands of errors into the near-certain regime ($p \ge 0.95$). (c) Confident errors concentrate disproportionately in long-tail tiers ($s_{\text{pop}} \in [10, 10^4)$).}
\label{fig:empirical_dynamics}
\end{figure}

Figure~\ref{fig:empirical_dynamics} illustrates this multi-faceted degradation across 22,267 queries. In Figure~\ref{fig:reliability}, base models adhere closely to the ideal diagonal ($y=x$), while aligned models show severe overconfidence across predicted probabilities. In Figure~\ref{fig:pbar_dist_main}, sequence confidence distributions ($\bar{p}$) confirm that unaligned base errors concentrate in low-confidence regions, whereas post-training alignment forces error mass into extreme certainty ($p \ge 0.95$). In Figure~\ref{fig:pop_tiers}, error rates across Wikipedia monthly pageview tiers in PopQA ($s_{\text{pop}}$) reveal that confident errors peak in the mid-to-long tail tiers ($s_{\text{pop}} \in [10, 10^4)$). While base models assign low probabilities to unfamiliar tail entities, aligned models allocate near-certain probabilities ($p \ge 0.95$) to fabricated completions. Disaggregated per-benchmark breakdowns appear in Table~\ref{tab:app_extended_breakdown} (Appendix~\ref{app:extended_breakdown_sec}), and capacity scaling analyses across 7B to 14B regimes appear in Figure~\ref{fig:app_scale} (Appendix~\ref{app:popularity_scale}).

\subsection{Persistence of Confident Errors under Decoding Perturbations}
\label{sec:persistence}

A relevant question is whether Gate B errors represent stochastic sampling noise or stable representational attractors. We evaluate response stability by sampling 10 independent completions per query at $T=0.7$ with top-$p=0.9$ across all Gate B instances.

The empirical results show that 68.4\% of Gate B errors in aligned models are rigid, with repeated samplings reproducing the identical fabricated entity. This high consistency causes uncertainty detection via semantic entropy \citep{kuhn2023semantic} and self-consistency to fail. On base models, semantic entropy discriminates between correct and incorrect answers with an AUROC of 0.78; on instruction-tuned models, semantic entropy AUROC drops to 0.51, barely exceeding random guessing. The model asserts false entities with the same internal agreement as factual truths (temperature sweeps and response stability curves appear in Table~\ref{tab:app_temperature_ablation} and Figure~\ref{fig:app_stability} in Appendix~\ref{app:stochastic_freezing}).

\subsection{Disentangling Model Weights from Formatting Templates}
\label{sec:disentangle}

We test whether overconfidence stems from conversational chat templates by comparing three conditions across all 22,267 queries, namely (1)~\textbf{Base + Few-Shot}, where base models use few-shot prefixes; (2)~\textbf{Instruct + Chat Template}, where aligned models use official chat templates; and (3)~\textbf{Instruct + Bare Completion}, where aligned models receive bare completion prefixes identical to Condition 1, stripping all chat wrappers (the complete open-science causal ladder tracing Base $\to$ SFT $\to$ DPO $\to$ RLVR appears in Table~\ref{tab:app_causal_ladder} and Appendix~\ref{app:causal_ladder_sec}).

\begin{table}[t]
\centering
\small
\caption{\textbf{Causal disentanglement of chat templates versus model weights.} Aligned models retain high error inflation even under bare completion prompts.}
\label{tab:causal_ablation}
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{llccc}
\toprule
\textbf{Model Family} & \textbf{Evaluation Condition} & \textbf{Gate B Count} & \textbf{Gate B (\%)} & \textbf{Inflation vs. Base} \\
\midrule
\multirow{3}{*}{Mistral-7B} & C1: Base Few-Shot & 63 & 0.28\% & 1.0$\times$ \\
 & C2: Instruct Chat Template & 1,630 & 7.32\% & 25.9$\times$ \\
 & C3: Instruct Bare Completion & 864 & 3.88\% & \textbf{13.7$\times$} \\
\midrule
\multirow{3}{*}{LLaMA-3-8B} & C1: Base Few-Shot & 18 & 0.08\% & 1.0$\times$ \\
 & C2: Instruct Chat Template & 637 & 2.86\% & 35.4$\times$ \\
 & C3: Instruct Bare Completion & 108 & 0.48\% & \textbf{6.0$\times$} \\
\midrule
\multirow{3}{*}{Qwen3-8B} & C1: Base Few-Shot & 92 & 0.41\% & 1.0$\times$ \\
 & C2: Instruct Chat Template & 924 & 4.15\% & 10.0$\times$ \\
 & C3: Instruct Bare Completion & 378 & 1.70\% & \textbf{4.1$\times$} \\
\bottomrule
\end{tabular}%
}
\end{table}

Table~\ref{tab:causal_ablation} shows that stripping chat formatting reduces Gate B errors from Condition 2 levels, but Condition 3 still retains a 4.1$\times$ to 13.7$\times$ error inflation over base models (e.g., 864 errors on Mistral-7B vs. 63 in base; 6.0$\times$ on LLaMA-3-8B). These measurements establish that prompt formatting contributes to superficial confidence, but internal parameter changes in model weights account for the dominant portion of overconfidence.


==> hce_arxiv/sections/04_representation_dynamics.tex <==
\section{Internal Representation Dynamics of Confident Errors}
\label{sec:mechanisms}

\subsection{Layer-Wise Probing with the Logit Lens}
\label{sec:logit_lens}

To trace where overconfidence originates within the transformer architecture, we probe intermediate representations using the Logit Lens \citep{belrose2023eliciting}. For a model with $L$ layers, let $h_t^{(l)} \in \mathbb{R}^d$ denote the hidden activation at layer $l \in \{1, \dots, L\}$ at output position $t$. We project $h_t^{(l)}$ onto the vocabulary $\mathcal{V}$ using the final layer normalization $\text{RMSNorm}$ and the pre-trained unembedding matrix $W_U \in \mathbb{R}^{|\mathcal{V}| \times d}$:
\begin{equation}
p_t^{(l)} = \text{softmax}\left( W_U \cdot \text{RMSNorm}\left(h_t^{(l)}\right) \right)
\label{eq:logit_lens}
\end{equation}
This projection yields a layer-wise probability distribution $p_t^{(l)}$ over vocabulary tokens without training external probes that could introduce auxiliary learning artifacts.

\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/fig3a_commitment.pdf}
    \caption{Commitment depth ($l^*$).}
    \label{fig:commitment}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/fig3b_margin.pdf}
    \caption{Late margin expansion.}
    \label{fig:late_margin}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/fig3c_submergence.pdf}
    \caption{Target token suppression.}
    \label{fig:gold_rank}
\end{subfigure}
\caption{\textbf{Internal representation dynamics on high-confidence completions} (\texttt{Mistral-7B}, all cohorts conditioned on terminal $p \ge 0.95$). (a) Commitment depth ($l^*$). Token predictions stabilize strictly in late layers ($l^*/L \ge 0.85$), showing early commitment does not hold for factual errors. (b) Late-layer margin expansion. Logit margins hover near zero through intermediate layers before expanding sharply in late layers ($l/L \ge 0.85$). (c) Target token suppression. Correct entity tokens drop deep into the vocabulary on confident factual errors ($<4\%$ top-1 recall vs.\ $>94\%$ for correct completions).}
\label{fig:mechanistic_lens}
\vspace{-8pt}
\end{figure}

To dissect the representation dynamics of extreme overconfidence, we condition our layer-wise analysis on completions producing high terminal confidence ($p \ge 0.95$). We compare \textbf{Gate A} (confident correct completions) and \textbf{Gate B} (rigid, confident incorrect completions verified across $k \ge 5$ samplings). In base models, where Gate B errors are exceptionally rare (0.4\%, 97 instances), we evaluate all instances alongside 500 sampled Gate A instances; in instruction models, we sample 500 instances per gate.

We evaluate whether early commitment, positing that transformers resolve factual associations in early layers \citep{geva2023dissecting}, holds across factual errors. Let $l^*$ denote the earliest layer where the top-1 predicted token permanently matches the final token. As shown in Figure~\ref{fig:commitment}, across all lineages the commitment depth satisfies $l^*/L \ge 0.85$ (layers 27--31 for 32-layer models). Across the first 80\% of layers ($l/L < 0.85$), intermediate representations maintain diffuse distributions and low match rates ($<25\%$), demonstrating the inapplicability of early commitment to factual retrieval errors (extended layer-wise projections and match statistics across architectures appear in Table~\ref{tab:app_logit_lens} and Figure~\ref{fig:app_layerwise_commitment} in Appendix~\ref{app:logit_lens_sec}).

Because both cohorts are conditioned on reaching terminal $p \ge 0.95$, their commitment trajectories track closely throughout intermediate depths (Figure~\ref{fig:commitment}). These overlapping trajectories reveal that when an aligned model manufactures a confident hallucination, its internal representations exhibit no early warning signal; false predictions lock into place through the same late-stage stabilization process as factual recall.

\subsection{Overconfidence Emerges in Late Layers}
\label{sec:late_layers}

We examine the layer-wise trajectory of decision entropy $\mathcal{H}(P_l)$ and top-1 logit margin $M_{1,l}$, defined as
\begin{equation}
\mathcal{H}(P_l) = -\sum_{v \in \mathcal{V}} p^{(l)}(v) \ln p^{(l)}(v), \qquad M_{1,l} = z_{(1)}^{(l)} - z_{(2)}^{(l)}
\label{eq:margin_entropy}
\end{equation}
where $z_{(1)}^{(l)}$ and $z_{(2)}^{(l)}$ denote the largest and second-largest unnormalized logits at layer $l$.

Figure~\ref{fig:late_margin} tracks this progression. Across layers 1 to 26 ($l/L < 0.85$), logit margins hover near zero ($M_l \le 0.3$) and entropy remains high ($\mathcal{H} > 2.0$ nats) across all cohorts, reflecting widespread ambiguity. In late layers ($l/L \ge 0.85$), margins expand past 4.0 points within three layers, collapsing entropy to zero. Because both cohorts in Figure~\ref{fig:late_margin} are conditioned on reaching terminal $p \ge 0.95$, their margins exhibit an identical late-stage surge. However, as established in Section~\ref{sec:empirical}, while base models restrict such extreme margin expansion to rare instances (0.4\%, 97 cases), post-training alignment forces thousands of confident factual errors (1,366 in Mistral-7B, 2,061 in Qwen3-14B) into this same severe expansion.

\subsection{Target Token Suppression and Vocabulary Fragmentation}
\label{sec:submergence}

While winning tokens in both Gate A and Gate B lock late with high margins, tracking gold entity tokens across layers (Figure~\ref{fig:gold_rank}) uncovers the true divergence. On Gate A, the gold token holds rank 1 in 94.4\% of instances ($>98\%$ in top-3). On Gate B, the gold token is substantially suppressed, with top-1 recall dropping to 3.8\% in Instruct and 4.1\% in Base, and sinking below rank 50 in over 35\% of cases (disaggregated recall trajectories across datasets appear in Table~\ref{tab:app_gold_rank_by_dataset} and Figure~\ref{fig:app_gold_rank_recall} in Appendix~\ref{app:gold_rank_sec}).

Furthermore, BPE tokenization fragments rare entities into multiple low-frequency subwords. Once late-layer margin expansion locks onto an incorrect initial token, autoregressive decoding continues along the hallucinated trajectory. Linear probes trained on intermediate hidden states corroborate that representations do not covertly retain the correct entity token (Table~\ref{tab:app_linear_probes} in Appendix~\ref{app:linear_probes_sec}). Thus, confident errors do not stem from near-miss confusion; rather, correct entity tokens are suppressed deep within the vocabulary while post-training alignment elevates an erroneous token to extreme certainty.

\subsection{Limits of Inference-Time Interventions}
\label{sec:test_time_limits}

Given that overconfidence emerges late, we examine whether test-time decoding adjustments can eliminate Gate B errors without retraining. We evaluate five representative interventions on 4,422 queries, namely (1)~\textbf{Defensive System Prompting}, instructing the model to express uncertainty; (2)~\textbf{Iterative Self-Correction}, a two-turn re-evaluation protocol; (3)~\textbf{Self-Consistency Voting}, sampling 10 reasoning paths at $T=0.7$; (4)~\textbf{Layer-Contrastive Decoding (DoLa)}, contrasting intermediate and late layers \citep{chuang2024dola}; and (5)~\textbf{Entropy Thresholding}, thresholding sequence entropy.

\begin{table}[t]
\centering
\small
\caption{\textbf{Inference-time mitigation on LLaMA-3-8B-Instruct.} Interventions eliminate at most 8.3\% of confident errors under $\ge 97\%$ retention.}
\label{tab:test_time}
\vspace{-6pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\textbf{Inference-Time Defense} & \textbf{Gate B Count} & \textbf{Gate B Reduction} & \textbf{Correct Retention} & \textbf{Effective Trade-off} \\
\midrule
Standard Instruct Baseline & 324 & 0.0\% & 100.0\% & Baseline \\
Defensive System Prompting & 306 & 5.6\% & 65.2\% & Severe over-hedging \\
Iterative Self-Correction & 308 & 4.9\% & 81.4\% (1.9\% on LLaMA-3.1) & Corrupts valid answers \\
Self-Consistency (10 samples) & 302 & 6.8\% & 97.4\% & 68.4\% rigid errors \\
DoLa Layer-Contrastive & 297 & 8.3\% & 97.1\% & Late margin limits gain \\
Entropy Thresholding & 308 & 4.8\% & 97.0\% & Bypassed by overconfidence \\
\bottomrule
\end{tabular}%
}
\end{table}

Deployable safety mechanisms must preserve valid capabilities; we enforce that interventions retain $\ge 97\%$ of correct answers. As shown in Table~\ref{tab:test_time}, all five test-time methods eliminate at most 4.8\% to 8.3\% of Gate B errors under this constraint. Defensive prompting reduces Gate B errors by 5.6\% but degrades retention to 65.2\% through evasive hedging. Self-correction triggers excessive revision of valid answers, causing retention on LLaMA-3.1-8B to collapse to 1.9\%. DoLa achieves an 8.3\% reduction, but remains bounded because margin expansion already shifts activation trajectories by layer 24 (extended sweeps across layers and scaling factors appear in Table~\ref{tab:app_layer_contrastive} in Appendix~\ref{app:layer_contrastive_sec}). More broadly, comprehensive evaluations across four model lineages confirm that post-hoc detectors and selective abstention fail to isolate confident errors (Tables~\ref{tab:app_detection_auroc}, \ref{tab:app_selective_abstention}, \ref{tab:app_mitigation_master}, and Figure~\ref{fig:app_risk_coverage} in Appendix~\ref{app:detection_and_abstention}). These findings demonstrate that inference heuristics cannot undo parameter-level margin expansion; resolving the Alignment Paradox requires regularizing post-training objectives.


==> hce_arxiv/sections/05_bounded_mitigation.tex <==
\section{Mitigating Confident Errors via Bounded Margin Alignment}
\label{sec:mitigation}

\begin{table}[t]
\centering
\small
\caption{\textbf{Factorial matrix across model families under single-epoch tuning.} BDM-DPO safely suppresses early-stage overconfidence with zero degradation to baseline accuracy. (Single-epoch tuning precedes severe margin inflation; see Table~\ref{tab:epoch_progression} for multi-epoch stress tests).}
\label{tab:factorial_matrix}
\vspace{-6pt}
\renewcommand{\arraystretch}{0.88}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccc}
\toprule
\textbf{Starting Checkpoint} & \textbf{Optimization Objective} & \textbf{Acc (\%)} & \textbf{Gate A} & \textbf{Gate B} & \textbf{$\Delta$Gate B} & \textbf{Gate B / Errors} & \textbf{ECE} & \textbf{Reduction} \\
\midrule
\multirow{2}{*}{\textbf{Mistral-7B-SFT}} & Standard DPO & 45.2 & 8,120 & 1,180 & -- & 12.69\% & 0.224 & Baseline \\
 & BDM-DPO (Ours) & 45.4 & 8,204 & 1,118 & -62 & \textbf{11.99\%} & 0.218 & \textbf{-5.3\%} \\
\midrule
\multirow{2}{*}{\textbf{Mistral-7B-Instruct}} & Standard DPO & 47.6 & 8,973 & 1,630 & -- & 15.37\% & 0.282 & Baseline \\
 & BDM-DPO (Ours) & 47.6 & 9,012 & 1,591 & -39 & \textbf{15.01\%} & 0.279 & \textbf{-2.4\%} \\
\midrule
\multirow{2}{*}{\textbf{LLaMA-3-8B-SFT}} & Standard DPO & 48.2 & 9,450 & 102 & -- & 1.07\% & 0.142 & Baseline \\
 & BDM-DPO (Ours) & 48.3 & 9,510 & 91 & -11 & \textbf{0.95\%} & 0.138 & \textbf{-10.8\%} \\
\midrule
\multirow{2}{*}{\textbf{LLaMA-3-8B-Instruct}} & Standard DPO & 50.6 & 10,210 & 342 & -- & 3.24\% & 0.245 & Baseline \\
 & BDM-DPO (Ours) & 50.6 & 10,240 & 306 & -36 & \textbf{2.90\%} & 0.238 & \textbf{-10.5\%} \\
\bottomrule
\end{tabular}%
}
\vspace{-6pt}
\end{table}

\subsection{Theoretical Analysis of Unbounded Margin Growth}
\label{sec:theory}

We examine the mathematical mechanism that drives late-layer margin expansion during preference optimization. Consider the standard Direct Preference Optimization (DPO; \citealt{rafailov2023direct}) objective parameterized by policy $\pi_\theta$ and frozen reference policy $\pi_{\text{ref}}$:
{\setlength{\abovedisplayskip}{3pt}\setlength{\belowdisplayskip}{3pt}
\begin{equation}
\mathcal{L}_{\text{DPO}}(\theta) = -\mathbb{E}_{(x, y_w, y_l) \sim \mathcal{D}} \left[ \ln \sigma \left( \beta \ln \frac{\pi_\theta(y_w \mid x)}{\pi_{\text{ref}}(y_w \mid x)} - \beta \ln \frac{\pi_\theta(y_l \mid x)}{\pi_{\text{ref}}(y_l \mid x)} \right) \right]
\label{eq:dpo_loss}
\end{equation}}
Let $\Delta r_\theta(x, y_w, y_l) = \ln \frac{\pi_\theta(y_w \mid x)}{\pi_{\text{ref}}(y_w \mid x)} - \ln \frac{\pi_\theta(y_l \mid x)}{\pi_{\text{ref}}(y_l \mid x)}$ denote the implicit reward margin between preferred response $y_w$ and dispreferred response $y_l$.

\begin{theorem}[Unbounded Margin Divergence on Factual Errors]
\label{thm:unbounded_margin}
Let $(x, y_w, y_l)$ be a preference pair concerning a factual entity absent from the reference policy $\pi_{\text{ref}}$, such that $\pi_{\text{ref}}(y_w \mid x) \approx \pi_{\text{ref}}(y_l \mid x) \le \epsilon$. For any finite policy parameterization, the gradient of $\mathcal{L}_{\text{DPO}}$ with respect to the implicit margin $\Delta r_\theta$ satisfies:
{\setlength{\abovedisplayskip}{3pt}\setlength{\belowdisplayskip}{3pt}
\begin{equation}
\frac{\partial \mathcal{L}_{\text{DPO}}}{\partial \Delta r_\theta} = -\beta \sigma\left(-\beta \Delta r_\theta\right) < 0, \quad \forall \Delta r_\theta \in (-\infty, +\infty)
\label{eq:dpo_grad}
\end{equation}}
Because $\sigma'(\cdot) > 0$ for all finite arguments, gradient descent continually forces $\Delta r_\theta \to +\infty$. Lacking parametric factual representations in early layers, the policy minimizes the objective by scaling final unembedding logits, driving top-1 logit margin $M_1 \to \infty$ and decision entropy $\mathcal{H}(P_1) \to 0$.
\end{theorem}

Appendix~\ref{app:proofs} provides complete proofs. Theorem~\ref{thm:unbounded_margin} shows that lacking a saturation threshold, preference optimization drives margins toward infinity. If parametric factual knowledge remains invariant while $M_1$ diverges, the expected calibration error satisfies $\text{ECE}(\pi_\theta) \ge \text{ECE}(\pi_{\text{ref}}) + \Delta_{\text{rel}}$ (Corollary~\ref{cor:reliability_distortion} in Appendix~\ref{app:proofs}). Because branching between candidate entities concentrates at initial token $y_1$ with subsequent transitions near-deterministic ($p(y_t \mid x, y_{<t}) \approx 1, \forall t > 1$; Lemma~\ref{lem:first_token} in Appendix~\ref{app:proofs}), bounding the logit margin at $t=1$ bounds sequence confidence $\bar{p}$, curtailing Gate B escalation while preserving fluency.

\subsection{Bounded Dynamic Margin Alignment and BDM-DPO}
\label{sec:bdm_formulation}

Theorem~\ref{thm:unbounded_margin} and Lemma~\ref{lem:first_token} motivate enforcing a principled bound on margin growth during post-training. We define Bounded Dynamic Margin DPO (BDM-DPO) by introducing an entropy-dependent margin ceiling:
{\setlength{\abovedisplayskip}{3pt}\setlength{\belowdisplayskip}{3pt}
\begin{equation}
\mathcal{L}_{\text{BDM}}(\theta) = -\mathbb{E}_{(x, y_w, y_l)} \left[ \ln \sigma \left( \min \left( \beta \Delta r_\theta(x, y_w, y_l), \; M_{\max}(\mathcal{H}_{\text{ref}}) \right) \right) \right]
\label{eq:bdm_loss}
\end{equation}}
where $M_{\max}(\mathcal{H}_{\text{ref}}) = M_0 \exp\left( -\gamma \frac{\mathcal{H}(\pi_{\text{ref}}(\cdot \mid x))}{\ln |\mathcal{V}|} \right)$ dynamically bounds the margin ($M_0 = 3.8$, $\gamma = 1.0$; grid searches and $\beta$ sweeps appear in Tables~\ref{tab:app_ablation_grid} and \ref{tab:app_beta_sweep} in Appendix~\ref{app:ablation_grid_sec}). When the reference model is certain ($\mathcal{H}_{\text{ref}} \approx 0$), $M_{\max} \approx M_0$, permitting full optimization; when uncertain ($\mathcal{H}_{\text{ref}}$ high), $M_{\max}$ contracts to prevent ungrounded margin escalation (Algorithm~\ref{alg:bdm_dpo} in Appendix~\ref{app:algorithm}). Under moderate single-epoch tuning, implicit margins remain below $M_0$, matching standard DPO; under multi-epoch tuning, the dynamic ceiling engages to constrain margin growth.

\subsection{Empirical Evaluation on Factual Benchmarks}
\label{sec:experiments}

Across two model families (Mistral-7B, LLaMA-3-8B) and two alignment states (SFT, instruction checkpoints), single-epoch BDM-DPO preserves baseline accuracy (50.6\% on LLaMA-Instruct) while curtailing nascent Gate B errors by up to 10.8\% (Table~\ref{tab:factorial_matrix}; two-way ANOVA $p < 0.01$, eliminating 148 confident falsehoods across all 22,267 queries).

\begin{table}[t]
\centering
\small
\caption{\textbf{Multi-epoch dynamics on Mistral-7B across 10 DPO epochs.} BDM-DPO constrains unconstrained margin growth, eliminating up to 850 confident errors (-35.3\%) and preserving +4.7pp factual accuracy.}
\label{tab:epoch_progression}
\vspace{-6pt}
\renewcommand{\arraystretch}{0.88}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccrr}
\toprule
 & \multicolumn{4}{c}{\textbf{Standard DPO}} & \multicolumn{4}{c}{\textbf{BDM-DPO (Ours)}} & \multicolumn{3}{c}{\textbf{Mitigation Effect}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-12}
\textbf{Epoch} & \textbf{Acc (\%)} & \textbf{Gate B} & \textbf{$M_1$} & \textbf{ECE} & \textbf{Acc (\%)} & \textbf{Gate B} & \textbf{$M_1$} & \textbf{ECE} & \textbf{$\Delta$Gate B} & \textbf{Reduction} & \textbf{$\Delta$Acc} \\
\midrule
Epoch 1  & 47.6 & 1,630 & 3.61 & 0.282 & 47.6 & 1,591 & 3.60 & 0.279 & -39  & -2.4\%  & +0.0pp \\
Epoch 2  & 47.2 & 1,745 & 3.75 & 0.301 & 47.6 & 1,605 & 3.68 & 0.285 & -140 & -8.0\%  & +0.4pp \\
Epoch 3  & 46.8 & 1,890 & 3.92 & 0.324 & 47.5 & 1,612 & 3.71 & 0.291 & -278 & -14.7\% & +0.7pp \\
Epoch 5  & 45.8 & 2,045 & 4.12 & 0.354 & 47.5 & 1,610 & 3.74 & 0.298 & -435 & -21.3\% & +1.7pp \\
Epoch 8  & 43.8 & 2,409 & 4.38 & 0.391 & \textbf{47.6} & \textbf{1,559} & \textbf{3.78} & \textbf{0.332} & \textbf{-850} & \textbf{-35.3\%} & \textbf{+3.8pp} \\
Epoch 10 & 42.9 & 2,137 & 4.51 & 0.410 & \textbf{47.6} & \textbf{1,480} & \textbf{3.77} & \textbf{0.363} & \textbf{-657} & \textbf{-30.7\%} & \textbf{+4.7pp} \\
\bottomrule
\end{tabular}%
}
\vspace{-6pt}
\end{table}

Under 10-epoch stress tests on Mistral-7B (Table~\ref{tab:epoch_progression}), standard DPO expands margins from $M_1 = 3.61$ to $4.51$, increasing Gate B errors by 49.2\% (to 2,409 at Epoch 8) while factual accuracy drops from 47.6\% to 43.8\%. In contrast, BDM-DPO caps $M_1 \le 3.80$, eliminating 850 confident errors (-35.3\%) while preserving 47.6\% accuracy (+3.8pp gain). By Epoch 10, Gate B errors drop to 1,480 (below the 1,615 base checkpoint), with +4.7pp accuracy and an ECE of 0.363 vs. 0.410 (longitudinal curves appear in Table~\ref{tab:app_multiepoch_cross} and Figure~\ref{fig:app_epoch_progression} in Appendix~\ref{app:multiepoch_cross_sec}).

\subsection{Cross-Lineage and Ablation Dynamics}
\label{sec:ablation_dynamics}

On LLaMA-3.1-SFT, standard DPO inflates $M_1$ from 1.766 to 1.855, increasing Gate B errors by 29.4\% (102 to 132), whereas BDM-DPO suppresses them to 94 (28.8\% reduction; replicates on Anthropic HH-RLHF, Table~\ref{tab:app_dataset_robust} in Appendix~\ref{app:dataset_robust_sec}). Qwen3-8B acts as a negative control: with high initial entropy ($\mathcal{H} = 1.65$), DPO shows no runaway margin growth ($M_1 \approx 2.20$), and BDM-DPO remains neutral (ratio 1.034). Reference-free SimPO \citep{meng2024simpo} degrades accuracy to 45.4\% while Gate B errors reach 1,687 (Table~\ref{tab:app_simpo_eval} in Appendix~\ref{app:cross_paradigm_sec}), confirming the stabilizing role of the reference anchor. Bounded margin alignment also restores detector separability on frozen checkpoints (Table~\ref{tab:app_detector_restoration} in Appendix~\ref{app:detector_restoration_sec}).

\subsection{Preserving General Reasoning Capabilities}
\label{sec:reasoning_capabilities}

On general reasoning benchmarks (MMLU, GSM8K, ARC-Challenge; \citealt{hendrycks2020measuring,cobbe2021gsm8k,clark2018think}), standard DPO degrades MMLU from 62.69\% to 61.76\% ($p < 10^{-4}$). In contrast, BDM-DPO preserves MMLU at 62.70\% ($p = 0.63$), gains +2.04pp on GSM8K (51.55\% vs. 49.51\%), and matches ARC-Challenge at 63.65\% (Table~\ref{tab:downstream_benchmarks} in Appendix~\ref{app:extended_bdm_dpo}).


==> hce_arxiv/sections/06_discussion_conclusion.tex <==
\section{Discussion and Conclusion}
\label{sec:conclusion}

The Alignment Paradox arises from unbounded preference gradients interacting with human preferences that reward assertive completions \citep{sharma2023towards}. Because gradient pressure persists across all finite margins, post-training alignment inflates late-layer margins on erroneous completions, forcing ungrounded assertions into extreme confidence regimes ($p \ge 0.95$) that bypass selective prediction and deferral filters \citep{geifman2017selective,kamath2020selective}. Because inference-time defenses achieve at most an 8.3\% error reduction under retention constraints, mitigating confident hallucinations requires training-time regularization.

These findings establish bounded margin optimization as a principled remedy for preference alignment. Instantiated as BDM-DPO, dynamically capping margin expansion eliminates up to 850 confident errors (35.3\% reduction) across 22,267 queries while preserving reasoning capabilities, curtailing associative drift and pseudologia fantastica without disrupting fluency (Table~\ref{tab:app_case_studies} and Appendix~\ref{app:qualitative_studies}). Because unconstrained margin growth affects preference objectives generally, extending dynamic bounds across broader post-training pipelines offers a principled path toward reliable alignment.

